Max-Min Grouped Bandits

In this paper, we introduce a multi-armed bandit problem termed max-min grouped bandits, in which the arms are arranged in possibly-overlapping groups, and the goal is to find the group whose worst arm has the highest mean reward. This problem is of interest in applications such as recommendation systems and resource allocation, and is also closely related to widely-studied robust optimization problems. We present two algorithms based successive elimination and robust optimization, and derive upper bounds on the number of samples to guarantee finding a max-min optimal or near-optimal group, as well as an algorithm-independent lower bound. We discuss the degree of tightness of our bounds in various cases of interest, and the difficulties in deriving uniformly tight bounds.

==> preamble.tex <==
% \usepackage[T1]{fontenc}
% \usepackage[utf8]{inputenc}
% \usepackage{amsthm}
% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{graphicx}
% \usepackage{dsfont}
% %\usepackage{cite}
% \usepackage{amsmath}
% \usepackage{array}
% \usepackage{multirow}
% \usepackage{caption}
% \usepackage{color}
% \usepackage{multicol}

\theoremstyle{plain}
\newtheorem{claim}{\protect\claimname}
\theoremstyle{plain}
\newtheorem{prop}{\protect\propositionname}
\theoremstyle{plain}
\newtheorem{lem}{\protect\lemmaname}
\theoremstyle{plain}
\newtheorem{thm}{\protect\theoremname}
\theoremstyle{plain}
\newtheorem{cor}{\protect\corollaryname}  
\theoremstyle{definition}
\newtheorem{defn}{\protect\definitionname}
\theoremstyle{definition}
\newtheorem{assump}{\protect\assumptionname}
\theoremstyle{definition}
\newtheorem{rem}{\protect\remarkname}

\makeatother
  
\usepackage{babel} 

\providecommand{\claimname}{Claim}
\providecommand{\lemmaname}{Lemma}
\providecommand{\propositionname}{Proposition}
\providecommand{\theoremname}{Theorem}
\providecommand{\corollaryname}{Corollary} 
\providecommand{\definitionname}{Definition}
\providecommand{\assumptionname}{Assumption}
\providecommand{\remarkname}{Remark}

\newcommand{\overbar}[1]{\mkern 1.25mu\overline{\mkern-1.25mu#1\mkern-0.25mu}\mkern 0.25mu}
\newcommand{\overbarr}[1]{\mkern 3.5mu\overline{\mkern-3.5mu#1\mkern-0.75mu}\mkern 0.75mu}
\newcommand{\mytilde}[1]{\mkern 0.5mu\widetilde{\mkern-0.5mu#1\mkern-0mu}\mkern 0mu}
\newcommand{\mytildee}[1]{\mkern 1.5mu\widetilde{\mkern-1.5mu#1\mkern-0mu}\mkern 0mu}
  
%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\minimize}{minimize} 
\newcommand{\openone}{\mathds{1}}

\newcommand{\todo}[1]{{\bf \color{red} [TODO] #1 }}

% Robust GP
\newcommand{\Dbar}{\overbar{D}}
\newcommand{\Rbar}{\overbar{R}}
\newcommand{\Runder}{\underline{R}}
\newcommand{\bdelta}{\boldsymbol{\delta}}
\newcommand{\kSE}{k_{\text{SE}}}
\newcommand{\kMat}{k_{\text{Mat\'ern}}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ecbar}{\overbar{\mathcal{E}}}

% Other
\newcommand{\GP}{{\rm GP}}
\newcommand{\gv}{\mathbf{g}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\wv}{\mathbf{w}}
\newcommand{\zvbar}{\overbar{\mathbf{z}}}

% Ranking and bandits
\newcommand{\thetamin}{\theta_{\mathrm{min}}}
\newcommand{\thetamax}{\theta_{\mathrm{max}}}
\newcommand{\Xhat}{\widehat{X}}
\newcommand{\Ghat}{\widehat{G}}
\newcommand{\jworst}{j_{\mathrm{worst}}}
\newcommand{\Actil}{\widetilde{\mathcal{A}}}
% \newcommand{\Stil}{\widetilde{S}}
\newcommand{\mab}{\texttt{mab}}
\newcommand{\cmp}{\texttt{btl}}
\newcommand{\pemab}{P_{\mathrm{e},\texttt{mab}}}
\newcommand{\pecmp}{P_{\mathrm{e},\texttt{btl}}}
\newcommand{\btheta}{\boldsymbol{\theta}}
\newcommand{\Alg}{\mathrm{ALG}}
\newcommand{\Geometric}{\mathrm{Geometric}}
\newcommand{\Ttotal}{T_{\mathrm{total}}}
\newcommand{\jsec}{j_{\mathrm{sec}}}

% NoisyDD
\newcommand{\NDhat}{\widehat{\mathrm{ND}}}
\newcommand{\PDhat}{\widehat{\mathrm{PD}}}
% \newcommand{\Dhat}{\widehat{\mathrm{D}}}
\newcommand{\Shat}{\widehat{S}}
\newcommand{\Ehat}{\widehat{E}}
\newcommand{\peid}{P_{\mathrm{e},1}^{(\mathrm{D})}}
\newcommand{\peind}{P_{\mathrm{e},1}^{(\mathrm{ND})}}
\newcommand{\peiid}{P_{\mathrm{e},2}^{(\mathrm{D})}}
\newcommand{\peiind}{P_{\mathrm{e},2}^{(\mathrm{ND})}}
\newcommand{\epsid}{\epsilon_{1}^{(\mathrm{D})}}
\newcommand{\epsind}{\epsilon_{1}^{(\mathrm{ND})}}
\newcommand{\epsiid}{\epsilon_{2}^{(\mathrm{D})}}
\newcommand{\epsiind}{\epsilon_{2}^{(\mathrm{ND})}}
\newcommand{\nid}{n_1^{(\mathrm{D})}}
\newcommand{\nind}{n_1^{(\mathrm{ND})}}
\newcommand{\niid}{n_2^{(\mathrm{D})}}
\newcommand{\niind}{n_2^{(\mathrm{ND})}}
\newcommand{\Npd}{N_{\mathrm{pos}}^{(\mathrm{D})}}
\newcommand{\Npnd}{N_{\mathrm{pos}}^{(\mathrm{ND})}}
\newcommand{\npd}{n_{\mathrm{pos}}^{(\mathrm{D})}}
\newcommand{\npnd}{n_{\mathrm{pos}}^{(\mathrm{ND})}}
\newcommand{\npos}{n_{\mathrm{pos}}}
\newcommand{\nneg}{n_{\mathrm{neg}}}
\newcommand{\Ntilpos}{\widetilde{N}_{\mathrm{pos}}}
% \newcommand{\Npos}{N_{\mathrm{pos}}}
% \newcommand{\Nneg}{N_{\mathrm{neg}}}
\newcommand{\Aid}{\mathcal{A}_{1,i}^{(\mathrm{D})}}
\newcommand{\Aind}{\mathcal{A}_{1,i}^{(\mathrm{ND})}}
\newcommand{\mutild}{\tilde{\mu}^{(\mathrm{D})}}
\newcommand{\mutilnd}{\tilde{\mu}^{(\mathrm{ND})}}

% OneDimBO

\newcommand{\diag}{\mathrm{diag}}
\newcommand{\cunder}{\underline{c}}
\newcommand{\cbar}{\overline{c}}
\newcommand{\mutil}{\widetilde{\mu}}
\newcommand{\sigmatil}{\widetilde{\sigma}}
\newcommand{\Tearly}{T_{\mathrm{early}}}
\newcommand{\Tlate}{T_{\mathrm{late}}}
\newcommand{\Rearly}{R_{\mathrm{early}}}
\newcommand{\Rlate}{R_{\mathrm{late}}}
\newcommand{\Ctil}{\widetilde{C}}
\newcommand{\ctil}{\widetilde{c}}
\newcommand{\ftil}{\widetilde{f}}
\newcommand{\UCB}{\mathrm{UCB}}
\newcommand{\LCB}{\mathrm{LCB}}
\newcommand{\UCBtil}{\widetilde{\mathrm{UCB}}}
\newcommand{\LCBtil}{\widetilde{\mathrm{LCB}}}
\newcommand{\Lctil}{\widetilde{\mathcal{L}}}

% NoisyAdaptiveGT

\newcommand{\nMIi}{n_{\mathrm{MI,1}}}
\newcommand{\nMIii}{n_{\mathrm{MI,2}}}
\newcommand{\nConc}{n_{\mathrm{Conc}}}
\newcommand{\nIndiv}{n_{\mathrm{Indiv}}}
\newcommand{\nHalving}{n_{\mathrm{Halving}}}
\newcommand{\kmax}{k_{\mathrm{max}}}
\newcommand{\ptil}{\widetilde{p}}
\newcommand{\elltil}{\widetilde{\ell}}
\newcommand{\Stil}{\widetilde{S}}
\newcommand{\ncheck}{\check{n}}

% SeparateGT

\newcommand{\cmean}{c_{\mathrm{mean}}}
\newcommand{\cvar}{c_{\mathrm{var}}}
\newcommand{\ccov}{c_{\mathrm{cov}}}
\newcommand{\cmax}{c_{\mathrm{max}}}

\newcommand{\dneg}{d_{\mathrm{neg}}}
\newcommand{\dpos}{d_{\mathrm{pos}}}
\newcommand{\Nneg}{N_{\mathrm{neg}}}
\newcommand{\Npos}{N_{\mathrm{pos}}}
\newcommand{\Nerr}{N_{\mathrm{err}}}
\newcommand{\alphaneg}{\alpha_{\mathrm{neg}}}
\newcommand{\alphapos}{\alpha_{\mathrm{pos}}}

\newcommand{\pej}{P_{\mathrm{e},j}}
\newcommand{\nusymm}{\nu_{\mathrm{symm}}}

% PooledData
\newcommand{\bpi}{\boldsymbol{\pi}}
\newcommand{\Nrm}{\mathrm{N}}
\newcommand{\CNrm}{\mathrm{CN}}

% ConverseGP
\newcommand{\vbar}{\overline{v}}

% GT_ICASSP

\newcommand{\pc}{P_{\mathrm{c}}}

% ActiveMRF

\newcommand{\lammin}{\lambda_{\mathrm{min}}}
\newcommand{\lammax}{\lambda_{\mathrm{max}}}
\newcommand{\missing}{\ast}
\newcommand{\pFAi}{p_{\mathrm{FA},i}}
\newcommand{\pMDi}{p_{\mathrm{MD},i}}
\newcommand{\bSigmatil}{\widetilde{\mathbf{\Sigma}}}
\newcommand{\mtil}{\widetilde{m}}
\newcommand{\Ptil}{\widetilde{P}}
\newcommand{\dmin}{d_{\mathrm{min}}}
\newcommand{\davg}{d_{\mathrm{avg}}}
\newcommand{\dmaxbar}{\overline{d}_{\mathrm{max}}}
\newcommand{\taumin}{\tau_{\mathrm{min}}}
\newcommand{\taumax}{\tau_{\mathrm{max}}}
\newcommand{\ntil}{\widetilde{n}}
\newcommand{\Ntil}{\widetilde{N}}
\newcommand{\Ncheck}{\check{N}}
\newcommand{\kbar}{\overbar{k}}

\newcommand{\mmin}{m_{\mathrm{min}}}
\newcommand{\mmax}{m_{\mathrm{max}}}

% PartialSBM
\newcommand{\ellv}{\boldsymbol{\ell}}
\newcommand{\Cieq}{C_{1,\mathrm{eq}}}
\newcommand{\Cidif}{C_{1,\mathrm{dif}}}
\newcommand{\Ctilde}{\tilde{C}}
\newcommand{\dbar}{\overline{d}}
\newcommand{\bsigma}{\boldsymbol{\sigma}}
\newcommand{\Poisson}{\mathrm{Poisson}}
\newcommand{\ktilde}{\tilde{k}}
 
% GT_ISIT
\newcommand{\Veq}{V_{\mathrm{eq}}}
\newcommand{\Vdif}{V_{\mathrm{dif}}}
\newcommand{\Vveq}{\mathbf{V}_{\mathrm{eq}}}
\newcommand{\Vvdif}{\mathbf{V}_{\mathrm{dif}}}
\newcommand{\veq}{v_{\mathrm{eq}}}
\newcommand{\vdif}{v_{\mathrm{dif}}}

%
% MultiMRI
%
\newcommand{\bpsi}{\boldsymbol{\psi}}

%
% Group testing 
%
\newcommand{\Hg}{\mathrm{Hypergeometric}}
\newcommand{\TV}{\mathrm{TV}}
\newcommand{\dTV}{d_{\mathrm{TV}}}

%
% Graphical model selection
%
\newcommand{\Gbar}{\overbar{G}}
\newcommand{\Mbar}{\overbar{M}}
\newcommand{\qmax}{q_{\mathrm{max}}}

%
% Community detection
%
\newcommand{\Bi}{\mathrm{Binomial}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ev}{\mathbf{E}}

%
% Support recovery
%
\newcommand{\Sbar}{\overbar{S}}
\newcommand{\sbar}{\overbar{s}}

%\newcommand{\Wdif}{W_{\mathrm{dif}}}
%\newcommand{\Weq}{W_{\mathrm{eq}}}
%\newcommand{\wdif}{w_{\mathrm{dif}}}
%\newcommand{\weq}{w_{\mathrm{eq}}}

\newcommand{\Sdif}{S_{\mathrm{dif}}}
\newcommand{\Seq}{S_{\mathrm{eq}}}
\newcommand{\sdif}{s_{\mathrm{dif}}}
\newcommand{\sdifbar}{\overbar{s}_{\mathrm{dif}}}
\newcommand{\seqbar}{\overbar{s}_{\mathrm{eq}}}
\newcommand{\seq}{s_{\mathrm{eq}}}
\newcommand{\sdifhat}{\hat{s}_{\mathrm{dif}}}
\newcommand{\sdifx}{\overbar{s} \backslash s}
\newcommand{\seqx}{\overbar{s} \cap s}

\newcommand{\Xvdif}{\mathbf{X}_{\overbar{s} \backslash s}}
\newcommand{\Xveq}{\mathbf{X}_{\overbar{s} \cap s}}
\newcommand{\Xvdifo}{\mathbf{X}_{s \backslash \overbar{s}}}
\newcommand{\xvdif}{\mathbf{x}_{\overbar{s} \backslash s}}
\newcommand{\xveq}{\mathbf{x}_{\overbar{s} \cap s}}
\newcommand{\xveqo}{\mathbf{x}_{s \backslash \overbar{s}}}

\newcommand{\Ord}{\mathcal{O}}
\newcommand{\Yctil}{\widetilde{\mathcal{Y}}}

\newcommand{\dmax}{d_{\mathrm{max}}}
\newcommand{\dH}{d_{\mathrm{H}}}

\newcommand{\jeq}{j_{\mathrm{eq}}}
\newcommand{\jdiff}{j_{\mathrm{dif}}}

\newcommand{\Zhat}{\hat{Z}}
\newcommand{\Zhatmax}{\hat{Z}_{\mathrm{max}}}
\newcommand{\zdiff}{z_{\mathrm{dif}}}
\newcommand{\zcomm}{z_{\mathrm{eq}}}

\newcommand{\bmin}{b_{\mathrm{min}}}
\newcommand{\Bmin}{\beta_{\mathrm{min}}}
\newcommand{\bmax}{b_{\mathrm{max}}}
\newcommand{\sigbeta}{\sigma_{\beta}}
\newcommand{\siglv}{\sigma_{\sdif}}
%\newcommand{\Tr}{\mathrm{Tr}}

%\newcommand{\sign}{\mathrm{sign}}
\newcommand{\SNRdB}{\mathrm{SNR}_{\mathrm{dB}}}

\newcommand{\Weq}{W_{\mathrm{eq}}}
\newcommand{\Wdif}{W_{\mathrm{dif}}}
\newcommand{\weq}{w_{\mathrm{eq}}}
\newcommand{\wdif}{w_{\mathrm{dif}}}
\newcommand{\feq}{f_{\mathrm{eq}}}
\newcommand{\fdif}{f_{\mathrm{dif}}}

\newcommand{\bgood}{b_{\mathrm{good}}}
\newcommand{\bbad}{b_{\mathrm{bad}}}

\newcommand{\btil}{\widetilde{b}}
\newcommand{\betatil}{\widetilde{\beta}}
\newcommand{\betatileq}{\widetilde{\beta}_{\mathrm{eq}}}
\newcommand{\betatildif}{\widetilde{\beta}_{\mathrm{dif}}}
\newcommand{\btileq}{\widetilde{b}_{\mathrm{eq}}}
\newcommand{\btildif}{\widetilde{b}_{\mathrm{dif}}}
\newcommand{\stileq}{\widetilde{s}_{\mathrm{eq}}}
\newcommand{\stildif}{\widetilde{s}_{\mathrm{dif}}}
\newcommand{\pieq}{\pi_{\mathrm{eq}}}
\newcommand{\pidif}{\pi_{\mathrm{dif}}}
\newcommand{\Sdifhat}{\hat{S}_{\mathrm{dif}}}

\newcommand{\Bcfano}{\mathcal{B}'_{\mathrm{Fano}}}

\newcommand{\Sceq}{\mathcal{S}_{\mathrm{eq}}}
\newcommand{\Scdif}{\mathcal{S}_{\mathrm{dif}}}
\newcommand{\Nc}{\mathcal{N}}

%
% From MultiMRI
%
\newcommand{\Pv}{\mathbf{P}}
\newcommand{\Wvtil}{\widetilde{\mathbf{W}}}
\newcommand{\wtil}{\widetilde{w}}
\newcommand{\xvhat}{\hat{\mathbf{x}}}

%
% From Expanders_FOCS
%
\newcommand{\Bernoulli}{\mathrm{Bernoulli}}
\newcommand{\Binomial}{\mathrm{Binomial}}
\newcommand{\imtil}{\tilde{\imath}}
\newcommand{\SNR}{\mathrm{SNR}}

%
% From PaperBI
%
\newcommand{\CLM}{C_{\mathrm{LM}}}
\newcommand{\CSC}{C_{\mathrm{SC}}}
\newcommand{\ISC}{I_{\mathrm{SC}}}
\newcommand{\CM}{C_{\mathrm{M}}}
\newcommand{\Qmin}{Q_{\mathrm{min}}}
\newcommand{\Phat}{\widehat{P}}

%
% From JournalSU
%
\newcommand{\pebar}{\overbar{P}_{\mathrm{e}}}
\newcommand{\petilde}{\tilde{p}_{\mathrm{e}}}
\newcommand{\pe}{P_{\mathrm{e}}}
\newcommand{\pen}{P_{\mathrm{e},n}}
\newcommand{\peQ}{P_{\mathrm{e},Q}} 
\newcommand{\pemax}{P_{\mathrm{e},\mathrm{max}}} 
\newcommand{\msg}{\mathsf{m}}

\newcommand{\Ez}{E_{0}}
\newcommand{\Er}{E_{\mathrm{r}}}
\newcommand{\Esp}{E_{\mathrm{sp}}}
\newcommand{\Eziid}{E_{0}^{\mathrm{iid}}}
\newcommand{\Ezcc}{E_{0}^{\mathrm{cc}}}
\newcommand{\Eohatcc}{\hat{E}_{0}^{\mathrm{cc}}}
\newcommand{\Eohatcost}{\hat{E}_{0}^{\mathrm{cost}}}
\newcommand{\Ezcost}{E_{0}^{\mathrm{cost}}}
\newcommand{\Ezcostprime}{E_{0}^{\mathrm{cost}^{\prime}}}
\newcommand{\Eriid}{E_{\mathrm{r}}^{\mathrm{iid}}}
\newcommand{\Ercc}{E_{\mathrm{r}}^{\mathrm{cc}}}
\newcommand{\Erccprime}{E_{\mathrm{r},12}^{\mathrm{cc}^{\prime}}}
\newcommand{\Ercost}{E_{\mathrm{r}}^{\mathrm{cost}}}
\newcommand{\Ercostprime}{E_{\mathrm{r}}^{\mathrm{cost}^{\prime}}}

\newcommand{\rcu}{\mathrm{rcu}}
\newcommand{\rcus}{\rcu_{s}}
\newcommand{\rcuss}{\rcu_{s}^{*}}
\newcommand{\rcusa}{\rcu_{s,a}^{*}}
\newcommand{\rcushat}{\widehat{\mathrm{rcu}}_{s}}
\newcommand{\rcusshat}{\widehat{\mathrm{rcu}}_{s}^{*}}
\newcommand{\alphasa}{\alpha^{\mathrm{iid}}}
\newcommand{\rcul}{\rcu_{\mathrm{L}}}
\newcommand{\rhohat}{\hat{\rho}}
\newcommand{\LM}{I_{\mathrm{LM}}}
\newcommand{\GMI}{I_{\mathrm{GMI}}}

\newcommand{\SetScc}{\mathcal{S}}
\newcommand{\SetSncc}{\mathcal{S}_{n}}
\newcommand{\SetSncost}{\mathcal{S}_{n}}
\newcommand{\SetSiid}{\mathcal{S}^{\mathrm{iid}}}
\newcommand{\SetScost}{\mathcal{S}}
\newcommand{\SetSniid}{\mathcal{S}_{n}^{\mathrm{iid}}}
\newcommand{\SetTcc}{\mathcal{T}}
\newcommand{\SetTiid}{\mathcal{T}^{\mathrm{iid}}}
\newcommand{\SetTcost}{\mathcal{T}}
\newcommand{\SetTncost}{\mathcal{T}_{n}}
\newcommand{\SetTncc}{\mathcal{T}_{n}}

\newcommand{\Miid}{M^{\mathrm{iid}}}
\newcommand{\Mcc}{M^{\mathrm{cc}}}
\newcommand{\Mcost}{M^{\mathrm{cost}}}
\newcommand{\Rcr}{R_{\mathrm{cr}}}
\newcommand{\Rcrs}{R_s^{\mathrm{cr}}}

\newcommand{\Fbar}{\overbar{F}}
\newcommand{\Funder}{\underline{F}}
\newcommand{\Gunder}{\underline{G}}
\newcommand{\PXv}{P_{\Xv}}
\newcommand{\qbar}{\overbar{q}}
\newcommand{\rbar}{\overbar{r}}
\newcommand{\rtilde}{\tilde{r}}
\newcommand{\atilde}{\tilde{a}}
\newcommand{\phitilde}{\tilde{\phi}}
\newcommand{\Mtilde}{\mytildee{M}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Rtilde}{\mytildee{R}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Wvtilde}{\widetilde{\mathbf{W}}}
\newcommand{\hover}{\overbar{h}}
\newcommand{\ubar}{\overbar{u}}
\newcommand{\Ubar}{\overbar{U}}
\newcommand{\xbarbar}{\overbar{\overbar{x}}}
\newcommand{\Xbarbar}{\overbar{\overbar{X}}}
\newcommand{\xbar}{\overbar{x}}
\newcommand{\Xbar}{\overbar{X}}
\newcommand{\xtilde}{\widetilde{x}}
\newcommand{\Xtilde}{\mytilde{X}}
\newcommand{\ybar}{\overbar{y}}
\newcommand{\zbar}{\overbar{z}}
\newcommand{\Zbar}{\overbar{Z}}
\newcommand{\thetabar}{\overbar{\theta}}

\newcommand{\av}{\mathbf{a}}
\newcommand{\Qv}{\mathbf{Q}}
\newcommand{\uvbar}{\overbar{\mathbf{u}}}
\newcommand{\uv}{\mathbf{u}}
\newcommand{\Uvbar}{\overbar{\mathbf{U}}}
\newcommand{\Uv}{\mathbf{U}}
%\newcommand{\vv}{\mathbf{v}}
\newcommand{\Vv}{\mathbf{V}}
\newcommand{\vvbar}{\overbar{\mathbf{v}}}
\newcommand{\xvbarbar}{\overbar{\overbar{\mathbf{x}}}}
\newcommand{\xvbar}{\overbar{\mathbf{x}}}
\newcommand{\xvtilde}{\widetilde{\mathbf{x}}}
\newcommand{\xv}{\mathbf{x}}
\newcommand{\Xvbarbar}{\overbar{\overbar{\mathbf{X}}}}
\newcommand{\Xvbar}{\overbar{\mathbf{X}}}
\newcommand{\Xvtilde}{\mytilde{\mathbf{X}}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Yvtilde}{\widetilde{\mathbf{Y}}}
\newcommand{\Xv}{\mathbf{X}}
\newcommand{\yv}{\mathbf{y}}
\newcommand{\Yv}{\mathbf{Y}}
\newcommand{\zv}{\mathbf{z}}
\newcommand{\Zv}{\mathbf{Z}}

\newcommand{\Yvs}{\mathbf{Y}_{\hspace*{-0.5ex}s}}
\newcommand{\Uvn}{\mathbf{U}_{\hspace*{-0.3ex}n}}
\newcommand{\Tvn}{\mathbf{T}_{\hspace*{-0.3ex}n}} 
\newcommand{\Vvi}{\mathbf{V}_{\hspace*{-0.3ex}1}} 
\newcommand{\Vvii}{\mathbf{V}_{\hspace*{-0.3ex}2}}
\newcommand{\Vvm}{\mathbf{V}_{\hspace*{-0.3ex}m}}
\newcommand{\Vvtilden}{\widetilde{\mathbf{V}}_{\hspace*{-0.3ex}n}}   
\newcommand{\QUn}{Q_{U\hspace*{-0.2ex},\hspace*{0.05ex}n}}
\newcommand{\QXgUn}{Q_{X|U\hspace*{-0.2ex},\hspace*{0.05ex}n}}
\newcommand{\QUXn}{Q_{UX\hspace*{-0.2ex},\hspace*{0.05ex}n}}
\newcommand{\Yvi}{\mathbf{Y}_{\hspace*{-0.5ex}1}}
\newcommand{\Yvii}{\mathbf{Y}_{\hspace*{-0.5ex}2}}
\newcommand{\Yvu}{\mathbf{Y}_{\hspace*{-0.5ex}u}}

\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\ic}{\mathcal{i}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}

\newcommand{\CC}{\mathbb{C}}
\newcommand{\EE}{\mathbb{E}}
\newcommand{\PP}{\mathbb{P}}
\newcommand{\RR}{\mathbb{R}}
\newcommand{\ZZ}{\mathbb{Z}}
\newcommand{\Qsf}{\mathsf{Q}}

%\newcommand{\al}{\{a_l\}}
%\newcommand{\rl}{\{r_l\}}
\newcommand{\rbarl}{\{\overbar{r}_l\}}
\newcommand{\defeq}{\triangleq}
\newcommand{\deq}{\stackrel{d}{=}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\erfcxi}{\mathrm{erfcx}_{1}}
\newcommand{\erfcx}{\mathrm{erfcx}}
\newcommand{\erfc}{\mathrm{erfc}}
\newcommand{\supp}{\mathrm{supp}}

\newcommand{\alphanl}{\alpha^{\mathrm{nl}}_n}
\newcommand{\alphal}{\alpha^{\mathrm{l}}_n}
\newcommand{\betanl}{\beta^{\mathrm{nl}}_n}
\newcommand{\betal}{\beta^{\mathrm{l}}_n}

\newcommand{\Es}{E_{\mathrm{s}}}
\newcommand{\EJ}{E_{\mathrm{J}}}
\newcommand{\EJi}{E_{\mathrm{J},1}}
\newcommand{\EJii}{E_{\mathrm{J},2}}

\newcommand{\Vmin}{V_{\mathrm{min}}}
\newcommand{\Vmax}{V_{\mathrm{max}}}

%
% From PaperExpurgated
%

\newcommand{\rcux}{\mathrm{rcux}}

\newcommand{\Eexiid}{E_{\mathrm{ex}}^{\mathrm{iid}}}
\newcommand{\Eexcc}{E_{\mathrm{ex}}^{\mathrm{cc}}}
\newcommand{\Eexhatcc}{\hat{E}_{\mathrm{ex}}^{\mathrm{cc}}}
\newcommand{\Eexcost}{E_{\mathrm{ex}}^{\mathrm{cost}}}
\newcommand{\Eexcostprime}{E_{\mathrm{ex}}^{\mathrm{cost}^{\prime}}}
\newcommand{\Exiid}{E_{\mathrm{x}}^{\mathrm{iid}}}
\newcommand{\Excc}{E_{\mathrm{x}}^{\mathrm{cc}}}
\newcommand{\Excost}{E_{\mathrm{x}}^{\mathrm{cost}}}
\newcommand{\Excoststar}{E_{\mathrm{x}}^{\mathrm{cost}^{*}}}
\newcommand{\Excostprime}{E_{\mathrm{x}}^{\mathrm{cost}^{\prime}}}
\newcommand{\Eex}{E_{\mathrm{ex}}}
\newcommand{\Ex}{E_{\mathrm{x}}}

\newcommand{\Pxbicm}{P_{X}^{\rm bicm}}

\newcommand{\Av}{\mathbf{A}}
\newcommand{\Bv}{\mathbf{B}}
\newcommand{\bv}{\mathbf{b}}
\newcommand{\mbar}{\overbar{m}}
\newcommand{\tv}{\mathbf{t}}

\newcommand{\Lsf}{\mathsf{L}}
\newcommand{\Csf}{\mathsf{C}}
\newcommand{\csf}{\mathsf{c}}
\newcommand{\Fsf}{\mathsf{F}}
\newcommand{\Tsf}{\mathsf{T}}

\newcommand{\brl}{\{\overbar{r}_l\}}

%
% From DocumentMU
%

\newcommand{\peobar}{\overbar{p}_{\mathrm{e},0}}
\newcommand{\peibar}{\overbar{p}_{\mathrm{e},1}}
\newcommand{\peiibar}{\overbar{p}_{\mathrm{e},2}}
\newcommand{\peiiibar}{\overbar{p}_{\mathrm{e},12}}
\newcommand{\peo}{P_{\mathrm{e},0}}
\newcommand{\pei}{P_{\mathrm{e},1}}
\newcommand{\peii}{P_{\mathrm{e},2}}
\newcommand{\peiii}{P_{\mathrm{e},12}}
\newcommand{\rcuo}{\mathrm{rcu}_{0}}
\newcommand{\rcui}{\mathrm{rcu}_{1}}
\newcommand{\rcuii}{\mathrm{rcu}_{2}}
\newcommand{\rcuiii}{\mathrm{rcu}_{12}}
\newcommand{\rcuiiiprime}{\mathrm{rcu}_{12}^{\prime}}
\newcommand{\rcuiiia}{\mathrm{rcu}_{12,1}}
\newcommand{\rcuiiib}{\mathrm{rcu}_{12,2}}

\newcommand{\Eiziid}{E_{0,1}^{\mathrm{iid}}}
\newcommand{\Eiiziid}{E_{0,2}^{\mathrm{iid}}}
\newcommand{\Eiiiziid}{E_{0,12}^{\mathrm{iid}}}
\newcommand{\Eiiiaziid}{E_{0,12,1}^{\mathrm{iid}}}
\newcommand{\Eiiibziid}{E_{0,12,2}^{\mathrm{iid}}}
\newcommand{\Eozcc}{E_{0,0}^{\mathrm{cc}}}
\newcommand{\Eizcc}{E_{0,1}^{\mathrm{cc}}}
\newcommand{\Eiizcc}{E_{0,2}^{\mathrm{cc}}}
\newcommand{\Eiiizcc}{E_{0,12}^{\mathrm{cc}}}
\newcommand{\Eiiizccprime}{E_{0,12}^{\mathrm{cc}^{\prime}}}
\newcommand{\Eiiizccpprime}{E_{0,12}^{\mathrm{cc}^{\prime\prime}}}
\newcommand{\Eiiiazcc}{E_{0,12,1}^{\mathrm{cc}}}
\newcommand{\Eiiibzcc}{E_{0,12,2}^{\mathrm{cc}}}
\newcommand{\Ehatiiiazcc}{\hat{E}_{0,12,1}^{\mathrm{cc}}}
\newcommand{\Eozcost}{E_{0,0}^{\mathrm{cost}}}
\newcommand{\Eizcost}{E_{0,1}^{\mathrm{cost}}}
\newcommand{\Eiizcost}{E_{0,2}^{\mathrm{cost}}}
\newcommand{\Eiiizcost}{E_{0,12}^{\mathrm{cost}}}
\newcommand{\Eiiiazcost}{E_{0,12,1}^{\mathrm{cost}}}
\newcommand{\Eiiibzcost}{E_{0,12,2}^{\mathrm{cost}}}
\newcommand{\Eiiizaccts}{E_{0,12,1}^{\text{cc-ts}}}

\newcommand{\Eiriid}{E_{\mathrm{r},1}^{\mathrm{iid}}}
\newcommand{\Eiiriid}{E_{\mathrm{r},2}^{\mathrm{iid}}}
\newcommand{\Eiiiriid}{E_{\mathrm{r},12}^{\mathrm{iid}}}
\newcommand{\Eiiiariid}{E_{\mathrm{r},12,1}^{\mathrm{iid}}}
\newcommand{\Eiiibriid}{E_{\mathrm{r},12,2}^{\mathrm{iid}}}
\newcommand{\Eorcc}{E_{\mathrm{r},0}^{\mathrm{cc}}}
\newcommand{\Eorccprime}{E_{\mathrm{r},0}^{\mathrm{cc}^{\prime}}}
\newcommand{\Eircc}{E_{\mathrm{r},1}^{\mathrm{cc}}}
\newcommand{\Eiircc}{E_{\mathrm{r},2}^{\mathrm{cc}}}
\newcommand{\Eiiircc}{E_{\mathrm{r},12}^{\mathrm{cc}}}
\newcommand{\Eiiiarcc}{E_{\mathrm{r},12,1}^{\mathrm{cc}}}
\newcommand{\Eiiibrcc}{E_{\mathrm{r},12,2}^{\mathrm{cc}}}
\newcommand{\Eorcost}{E_{\mathrm{r},0}^{\mathrm{cost}}}
\newcommand{\Eircost}{E_{\mathrm{r},1}^{\mathrm{cost}}}
\newcommand{\Eiircost}{E_{\mathrm{r},2}^{\mathrm{cost}}}
\newcommand{\Eiiircost}{E_{\mathrm{r},12}^{\mathrm{cost}}}
\newcommand{\Eiiiarcost}{E_{\mathrm{r},12,1}^{\mathrm{cost}}}
\newcommand{\Eiiibrcost}{E_{\mathrm{r},12,2}^{\mathrm{cost}}}
\newcommand{\Eiiirtilde}{\widetilde{E}_{\mathrm{r,12}}}
\newcommand{\Eiiirccts}{E_{\mathrm{r},12}^{\text{cc-ts}}}

\newcommand{\Wsu}{W^{\prime}}
\newcommand{\qsu}{q^{\prime}}
\newcommand{\RegLM}{\mathcal{R}_{\mathrm{LM}}}
\newcommand{\RegLMex}{\mathcal{R}_{\mathrm{ex}}}

\newcommand{\SetSccts}{\mathcal{S}^{\mathrm{ts}}}
\newcommand{\SetTocc}{\mathcal{T}_0}
\newcommand{\SetToncc}{\mathcal{T}_{0,n}}
\newcommand{\SetTicc}{\mathcal{T}_{1}}
\newcommand{\SetTiicc}{\mathcal{T}_{2}}
\newcommand{\SetTiiicc}{\mathcal{T}_{12}}
\newcommand{\SetTiiincc}{\mathcal{T}_{12,n}}
\newcommand{\SetTnucc}{\mathcal{T}_{\nu}}
\newcommand{\SetTnuccex}{\mathcal{T}_{\nu}^{\mathrm{ex}}}
\newcommand{\SetTiccex}{\mathcal{T}_{1}^{\mathrm{ex}}}
\newcommand{\SetTiiccex}{\mathcal{T}_{2}^{\mathrm{ex}}}
\newcommand{\SetTiiiccex}{\mathcal{T}_{12}^{\mathrm{ex}}}
\newcommand{\SetTiccts}{\mathcal{T}_{1}^{\mathrm{ts}}}
\newcommand{\SetTiiccts}{\mathcal{T}_{2}^{\mathrm{ts}}}
\newcommand{\SetTiiiccts}{\mathcal{T}_{12}^{\mathrm{ts}}}

\newcommand{\qv}{\mathbf{q}}
\newcommand{\Wv}{\mathbf{W}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Vc}{\mathcal{V}}

\newcommand{\Rsc}{R^{\mathrm{sc}}}
\newcommand{\Rmac}{R^{\mathrm{ex}}}
\newcommand{\Rosc}{R_{0}^{\mathrm{sc}}}
\newcommand{\Risc}{R_{1}^{\mathrm{sc}}}
\newcommand{\Rimac}{R_{1}^{\mathrm{ex}}}
\newcommand{\Riimac}{R_{2}^{\mathrm{ex}}}
\newcommand{\Usc}{U^{\mathrm{sc}}}
\newcommand{\Ucsc}{\mathcal{U}^{\mathrm{sc}}}
\newcommand{\Ximac}{X_{1}^{\mathrm{ex}}}
\newcommand{\Xcimac}{\mathcal{X}_{1}^{\mathrm{ex}}}
\newcommand{\Xiimac}{X_{2}^{\mathrm{ex}}}
\newcommand{\Xciimac}{\mathcal{X}_{2}^{\mathrm{ex}}}

\newcommand{\PrML}{\PP^{(\mathrm{ML})}}
\newcommand{\PrS}{\PP^{(\mathrm{S})}}
\newcommand{\PrGenie}{\PP^{(\mathrm{Genie})}}

%
% From MAC2OR
%
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\cv}{\mathbf{c}}
\newcommand{\Dv}{\mathbf{D}}
\newcommand{\Iv}{\mathbf{I}}
\newcommand{\iv}{\mathbf{i}}
\newcommand{\Fv}{\mathbf{F}}
\newcommand{\fv}{\mathbf{f}}
\newcommand{\Mv}{\mathbf{M}}
\newcommand{\Jv}{\mathbf{J}}
\newcommand{\Kv}{\mathbf{K}}
\newcommand{\kv}{\mathbf{k}}
\newcommand{\Lv}{\mathbf{L}}
\newcommand{\Rv}{\mathbf{R}}
\newcommand{\sv}{\mathbf{s}}
\newcommand{\Sv}{\mathbf{S}}
\newcommand{\Tv}{\mathbf{T}}
\newcommand{\bzero}{\boldsymbol{0}}
\newcommand{\bone}{\boldsymbol{1}}
\newcommand{\bmu}{\boldsymbol{\mu}}
\newcommand{\bphi}{\boldsymbol{\phi}}
\newcommand{\bgamma}{\boldsymbol{\gamma}}
\newcommand{\bTheta}{\boldsymbol{\Theta}}
\newcommand{\bOmega}{\boldsymbol{\Omega}}
\newcommand{\bSigma}{\boldsymbol{\Sigma}}
\newcommand{\bLambda}{\boldsymbol{\Lambda}}
\newcommand{\bPsi}{\boldsymbol{\Psi}}
\newcommand{\bDelta}{\boldsymbol{\Delta}}
\newcommand{\bell}{\boldsymbol{\ell}}
\newcommand{\Qinv}{\mathsf{Q}_{\mathrm{inv}}}

%
% From RefinementCC
%
\newcommand{\Wocc}{\mathcal{W}_{0}^{\mathrm{cc}}}
\newcommand{\Wosymm}{\mathcal{W}_{0}^{\mathrm{symm}}}
\newcommand{\Wsymm}{\mathcal{W}^{\mathrm{symm}}}
\newcommand{\Qocc}{\mathcal{Q}_{0}^{\mathrm{cc}}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\bxi}{\boldsymbol{\xi}}
\newcommand{\Ezxcc}{E_{0,x}^{\mathrm{cc}}}
\newcommand{\Ezxicc}{E_{0,x_{i}}^{\mathrm{cc}}}
\newcommand{\Rcrsa}{R_{s,a}^{\mathrm{cr}}}
